mPLUG-Owl2: Revolutionizing Multi-modal Large Language Model with Modality Collaboration

Multi-modal Large Language Models (MLLMs) have demonstrated impressive instruction abilities across various open-ended tasks. However, previous methods primarily focus on enhancing multi-modal capabilities. In this work, we introduce a versatile multi-modal large language model, mPLUG-Owl2, which effectively leverages modality collaboration to improve performance in both text and multi-modal tasks. mPLUG-Owl2 utilizes a modularized network design, with the language decoder acting as a universal interface for managing different modalities. Specifically, mPLUG-Owl2 incorporates shared functional modules to facilitate modality collaboration and introduces a modality-adaptive module that preserves modality-specific features. Extensive experiments reveal that mPLUG-Owl2 is capable of generalizing both text tasks and multi-modal tasks and achieving state-of-the-art performances with a single generic model. Notably, mPLUG-Owl2 is the first MLLM model that demonstrates the modality collaboration phenomenon in both pure-text and multi-modal scenarios, setting a pioneering path in the development of future multi-modal foundation models.

==> tables/ablation_moe.tex <==
% \begin{table}
% \centering
%     \tablestyle{7pt}{1.1} 
%     \def \w{15pt}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|c|cccc}
%         % \toprule
%         % \shline
%         Method     &  MAM  & VQAv2 & MMBench & Q-Bench & MMLU \\
%         \shline
%         LLaVA-1.5 \cite{}  &  & 78.5 & 62.7 & 58.7 & 50.4  \\
%         LLaVA-1.5 \cite{} & \checkmark & 78.8 \textbf{\color{red}{(+0.3)}} & 64.0 \textbf{\color{red}{(+1.3)}} & 59.5 \textbf{\color{red}{(+0.8)}} & 51.4 \textbf{\color{red}{(+1.0)}} \\
%         \hline
%         \modelname  &  & 76.2 & 63.8 & 61.3 & 51.8  \\
%         \modelname & \checkmark & xxxx & xxxx & xxxxx & xxxx  \\
%         % \shline
%         % \bottomrule
%     \end{tabular}
%     }
%     \caption{Effectiveness and generalization of Modality-Adaptive Module (MAM) across different approaches. Note that for LLaVA-1.5 \cite{}, we follow the original implementation use the input resolution of $336 \times 336$.}
%     \label{table:moe-ablation}
% \end{table}




\begin{table}[h]
\centering
    \tablestyle{7pt}{1.1} 
    \def \w{15pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|cccc}
        % \toprule
        % \shline
        \multirow{2}{*}{Method}   &  LLM Tuning   & \multirow{2}{*}{VQAv2} & \multirow{2}{*}{MMBench} & \multirow{2}{*}{Q-Bench} & \multirow{2}{*}{MMLU} \\
        & Method & & & &  \\
        \shline
        LLaVA-1.5 \cite{Liu2023LLava15}  & Full & 78.5 & 62.7 & 58.7 & 50.4  \\ 
        LLaVA-1.5 \cite{Liu2023LLava15}  & Freeze  & 70.6 \textbf{\color{deepgreen}{(-7.9)}} & 48.2 \textbf{\color{deepgreen}{(-14.5)}} & 32.6 \textbf{\color{deepgreen}{(-26.1)}} & 51.1 \textbf{\color{red}{(+0.7)}} \\ 
        LLaVA-1.5 \cite{Liu2023LLava15}  &  LoRA &  79.1 \textbf{\color{red}{(+0.6)}} & 65.0 \textbf{\color{red}{(+2.3)}} & 58.4 \textbf{\color{deepgreen}{(-0.3)}}  & 50.2 \textbf{\color{deepgreen}{(-0.2)}}  \\ \hline
        LLaVA-1.5 \cite{Liu2023LLava15} & Full w/ MAM &  78.8 \textbf{\color{red}{(+0.3)}} & 64.0 \textbf{\color{red}{(+1.3)}} & 59.5 \textbf{\color{red}{(+0.8)}} & 52.5 \textbf{\color{red}{(+2.1)}} \\
        LLaVA-1.5 \cite{Liu2023LLava15} & LoRA w/ MAM &  79.2 \textbf{\color{red}{(+0.7)}} & 66.0 \textbf{\color{red}{(+3.3)}} & 59.7 \textbf{\color{red}{(+1.0)}} & 52.0 \textbf{\color{red}{(+1.6)}} \\
        % \shline
        % \bottomrule
    \end{tabular}
    }
    % \caption{Effectiveness and generalization of Modality-Adaptive Module (MAM) across different approaches. Note that for LLaVA-1.5 \cite{}, we follow the original implementation use the input resolution of $336 \times 336$.}
    \caption{Illustration the phenomenon of modality collaboration and interference. For the LoRA version, we directly utilize the official checkpoint\protect\footnotemark, which might tuned carefully. We follow the original implementation using the input resolution of $336 \times 336$.}
    \vspace{-2ex}
    \label{table:moe-ablation}
\end{table}

\footnotetext{The checkpoint is recently released on October 27th, 2023.}
